A reduced-precision streaming SpMV architecture for Personalized PageRank on FPGA

Sparse matrix-vector multiplication is often employed in many data-analytic workloads in which low latency and high throughput are more valuable than exact numerical convergence. FPGAs provide quick execution times while offering precise control over the accuracy of the results thanks to reduced-precision fixed-point arithmetic. In this work, we propose a novel streaming implementation of Coordinate Format (COO) sparse matrix-vector multiplication, and study its effectiveness when applied to the Personalized PageRank algorithm, a common building block of recommender systems in e-commerce websites and social networks. Our implementation achieves speedups up to 6x over a reference floating-point FPGA architecture and a state-of-the-art multi-threaded CPU implementation on 8 different data-sets, while preserving the numerical fidelity of the results and reaching up to 42x higher energy efficiency compared to the CPU implementation.

==> code/scaling.tex <==
\begin{algorithm}
    \caption{Computing the scaling vector of \gls{ppr}}\label{alg:scaling}
    \begin{algorithmic}[1]
    \Function{Scaling}{$\mathbf{P}, \mathbf{\bar{d}}$}
        \LineComment{Blocks have $B$ elements and size $P\_SIZE$}
        \For{$i \gets 0, |V| / B$} 
            \State $dangling = \mathbf{\bar{d}}[i / (P\_SIZE / B)]$
        
            \For{$k \gets 0,\kappa$} 
                \For{$b \gets 0,B$} 
                    \State $d\_buffer[k, b] =$\par
                    \hskip\algorithmicindent$\mathbf{P}[k, i \cdot B + b] + dangling[(i \cdot B + j)\ \%\ P\_SIZE]$
                \EndFor
                \State $dangling\_vals[k, :] \pluseq sum(d\_buffer[k, :])$
            \EndFor
        \EndFor
        \State Return $\alpha \cdot dangling\_vals$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> tables/resources.tex <==
\renewcommand\theadalign{tl}
\renewcommand\theadfont{\bfseries}
% \setlength\tabcolsep{5pt}
% \renewcommand\theadgape{\Gape[10pt]}
% \renewcommand\cellgape{\Gape[10pt]}

\begin{table*}
\centering
\ra{1.1}
    \caption{Resource utilization and power consumption of our architecture. Floating point arithmetic greatly increases the use of DSPs and LUTs, while LUT utilization and clock frequency change linearly w.r.t bit-width. Intermediate bit-widths are omitted for brevity, but they show the same trends}
    \resizebox{1\linewidth}{!}{
	\begin{tabular}{@{}lllllllll@{}}
		\toprule
	% 2 Lines
% 	& \multirow{2}{*}{\thead{Bit-width}} & \multirow{2}{*}{\thead{BRAM}} & \multirow{2}{*}{\thead{DSP}} & \multirow{2}{*}{\thead{FF}} & \multirow{2}{*}{\thead{LUT}}  & \multirow{2}{*}{\thead{URAM}} &\multirow{2}{*}{\thead{Clock}} & \thead{Power\\Consumption}\\
    % 1 Line
	& \thead{Bit-width} & \thead{BRAM} & \thead{DSP} & \thead{FF} & \thead{LUT}  & \thead{URAM} & \thead{Clock} & \thead{Power Cons.}\\
	   
	    \midrule
    	% \textbf{Total resources} &  & 4320 & 6840 & 2364480 & 1182240 & 960 &  &  \\
    	
% 	    100K buffer
    	
		\textbf{Fixed-point} & 20 bits & 608 (14\%) & 272 (3\%) & 96197 (4\%) & 312202 (26\%) & 192 (20\%) & 220 MHz & 34 W \\
		 
		 & 26 bits & 608 (14\%) & 272 (3\%) & 96197 (4\%) & 455880 (38\%) & 192 (20\%) & 200 MHz & 35 W \\
		
		\textbf{Floating-point} & 32 bits & 608 (14\%) & 3298 (48\%) & 832114 (35\%) & 1061382 (89\%) & 256 (26\%) & 115 MHz & 40 W \\
		
% 		200K buffer

% 		\textbf{Fixed-point} & 20 bits & 672 (15\%) & 400 (5\%) & 104159 (4\%) & 351010 (29\%) & 384 (40\%) & 130 MHz & 34 W \\
		
		% & 22 bits & 672 (15\%) & 264 (3\%) & 178949 (7\%) & 452323 (38\%) & 384 (40\%) & 125 MHz & 34 W \\
		 
		% & 24 bits & 672 (15\%) & 400 (5\%) & 153884 (6\%) & 256653 (21\%) & 384 (40\%) & 120 MHz & 35 W \\
		 
% 		 & 26 bits & 672 (15\%) & 400 (5\%) & 177484 (7\%) & 492674 (41\%) & 384 (40\%) & 115 MHz & 35 W \\
		
% 		\textbf{Floating-point} & 32 bits & 608 (14\%) & 3298 (48\%) & 832149 (35\%) & 1061389 (89\%) & 512 (53\%) & 200 MHz & 40 W \\

		\bottomrule
	\end{tabular}
    }
    \label{tab:resources}
\end{table*}
